Slow Light in Metamaterial Waveguides

Metamaterials, which are materials engineered to possess novel optical properties, have been increasingly studied. The ability to fabricate metamaterials has sparked an interest in determining possible applications. We investigate using a metamaterial for boundary engineering in waveguides. A metamaterial-clad cylindrical waveguide is used to provide confinement for an optical signal, thereby increasing the local electromagnetic energy density. We show that metamaterial-clad waveguides have unique optical properties, including new modes, which we call hybrid modes. These modes have properties of both ordinary guided modes and surface plasmon-polariton modes. We show that for certain metamaterial parameters, the surface plasmon-polariton modes of a metamaterial-clad waveguide have less propagation loss than those of a metal-clad guide with the same permittivity. This low-loss mode is exploited for all-optical control of weak fields. Embedding three-level {\Lambda} atoms in the dielectric core of a metamaterial-clad waveguide allows the use of electromagnetically induced transparency to control an optical signal. Adjusting the pump field alters the group velocity of the signal, thereby controllably delaying pulses. Using the low-loss surface mode of a metamaterial-clad guide reduces losses by 20% over a metal cladding without sacrificing the group velocity reduction or confinement. In addition, we show that losses can be reduced by as much as 40% with sufficient reduction of the magnetic damping constant of the metamaterial. As this work aims for applications, practical considerations for fabricating and testing metamaterial-clad waveguides are discussed. An overview of the benefits and drawbacks for two different dielectric core materials is given. Also, a short discussion of other modes that could be used is given.

==> symbols.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
%Sample List of Symbols
%%%%%%%%%%%%%%%%%%%%%%%


\begin{tabbing}
Symbol~~~~~\= \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \parbox{5in}{Definition}\\

\addsymbol \mbox{U of C}: {University of Calgary}
\addsymbol {\epsilon_{0}}: {Permittivity of free space}
\addsymbol {\mu_{0}}: {Permeability of free space}
\addsymbol {\bm E}: {Electric field}
\addsymbol {\bm D}: {Electric displacement field}
\addsymbol {\bm B}: {Magnetic field}
\addsymbol {\bm H}: {Auxiliary magnetic field}
\addsymbol {\bm P}: {Electric polarization field}
\addsymbol {\tilde{\beta}}: {Complex propagation constant of a waveguide}
\addsymbol {\gamma_{j}}: {Complex transverse wavenumber in $j$th region of a waveguide}
\addsymbol {\beta}: {Dispersion of a mode in a waveguide}
\addsymbol {\alpha}: {Attenuation rate of a mode in a waveguide}
\addsymbol {R^{(n)}}: {$n$th order polarization response function}
\addsymbol {\chi^{(1)}}: {Linear electric susceptibility}
\addsymbol {\chi^{(n)}}: {Nonlinear electric susceptibility for $n\geq2$}
\addsymbol{\nabla^{2}}: {The Laplacian}
\addsymbol \mbox{EM}: {Electromagnetic}
\addsymbol \mbox{TM}: {Transverse Magnetic}
\addsymbol \mbox{TE}: {Transverse Electric}
\addsymbol \mbox{HE or EH}: {Modes of a cylindrical guide with no non-zero field components}
\addsymbol \mbox{EIT}: {Electromagnetically induced transparency}
\addsymbol \mbox{SPP}: {Surface plasmon-polariton}
\addsymbol \mbox{RE}: {Rare-earth}
\addsymbol {\Omega_{\text p}}: {Rabi frequency of the pump field driving the EIT atoms}
\addsymbol {\eta}: {Parameter used to control Rabi frequency of the pump field}
% .
% .
% .
% ALWAYS KEEP THE FOLLOWING LINE
\end{tabbing}

